Offboard 3D Object Detection from Point Cloud Sequences

While current 3D object recognition research mostly focuses on the real-time, onboard scenario, there are many offboard use cases of perception that are largely under-explored, such as using machines to automatically generate high-quality 3D labels. Existing 3D object detectors fail to satisfy the high-quality requirement for offboard uses due to the limited input and speed constraints. In this paper, we propose a novel offboard 3D object detection pipeline using point cloud sequence data. Observing that different frames capture complementary views of objects, we design the offboard detector to make use of the temporal points through both multi-frame object detection and novel object-centric refinement models. Evaluated on the Waymo Open Dataset, our pipeline named 3D Auto Labeling shows significant gains compared to the state-of-the-art onboard detectors and our offboard baselines. Its performance is even on par with human labels verified through a human label study. Further experiments demonstrate the application of auto labels for semi-supervised learning and provide extensive analysis to validate various design choices.

==> tex/abstract_v2.tex <==
In autonomous driving, sufficient and accurate 3D cuboid annotations is the fuel that powers machine learning based components, including perception, behavior prediction, path planning, etc. 
Such data becomes available at a tremendous cost in human labors, time and resources. In this paper, we propose a novel offboard 3D object detection pipeline (3D Auto Labeling) to generate high-quality cuboids and tracks from point cloud videos, for the purpose of automating 3D annotations. While current 3D object recognition research mostly focuses on the real-time, onboard scenario, the offboard space and its potentials are largely under-exploited, where more sophisticated models can be afforded and the models can leverage input data at a substantially extended horizon both spatially and temporally. Specifically, observing that different frames often capture complementary views of objects, we design a powerful framework to make better use of the temporal information, which consists of a multi-frame object detector and a novel object-centric auto labeling model that processes 4D object track data and outputs temporally consistent and high-quality boxes. Evaluated on the Waymo Open Dataset, our 3D Auto Labeling pipeline shows significant gains in detection, tracking and domain adaptation compared to the state-of-the-art onboard detectors as well as our own offboard baselines. Its performance is even on par with human annotators, based on our human label study. Further experiments demonstrate the promising application of auto labels for semi-supervised learning and provide extensive analysis to validate various design choices of the pipeline.


% While current 3D object recognition research mostly focuses on the real-time, onboard scenario, there are many offboard use cases of perception that are largely under-explored such as using machines to automatically generate high-quality 3D labels. Existing 3D object detectors fail to satisfy the high-quality requirement for offboard uses due to the limited input data and constraints on inference speed. In this paper, we propose a novel offboard 3D object detection pipeline using point cloud video data. Observing that different frames often capture complementary views of objects, we design the offboard detector to make use of the temporal frame data through both multi-frame object detection and a novel object-centric auto labeling model that processes 4D object track data to outputs temporally consistent and high-quality boxes. Evaluated on the Waymo Open Dataset, our pipeline named 3D Auto Labeling shows significant gains in detection, tracking and domain adaptation compared to the state-of-the-art onboard detectors and our own offboard baselines. Its performance is even on par with human labels verified through a human label study. Further experiments demonstrates the application of using auto labels for semi-supervised learning and provides extensive analysis to validate various designs of the pipeline.
